Velos: One-sided Paxos for RDMA applications

Modern data centers are becoming increasingly equipped with RDMA-capable NICs. These devices enable distributed systems to rely on algorithms designed for shared memory. RDMA allows consensus to terminate within a few microsecond in failure-free scenarios, yet, RDMA-optimized algorithms still use expensive two-sided operations in case of failure. In this work, we present a new leader-based consensus algorithm that relies solely on one-sided RDMA verbs. Our algorithm is based on Paxos, it decides in a single one-sided RDMA operation in the common case, and changes leader also in a single one-sided RDMA operation in case of failure. We implement our algorithm in the form of an SMR system named Velos, and we evaluated our system against the state-of-the-art competitor Mu. Compared to Mu, our solution adds a small overhead of approximately 0.6 microseconds in failure-free executions and shines during failover periods during which it is 13 times faster in changing leader.

==> pseudocode/og-nonabortable-paxos.tex <==
\begin{lstlisting}[columns=fullflexible,breaklines=true,keywords={while,if,else,return,do,for}, aboveskip=0pt, belowskip=0pt, float=ht! ,caption={ Algorithm for basic RPC-Paxos},label={alg:consensus-basic}] 
@\textbf{Proposers execute:}
upon <Init>:
    decided = False
    proposal = id
    proposed_value = @$\bot$@
    
propose(value):
    proposed_value = value
    while not decided:
        prepare()
        accept()
    
prepare():
    proposal = proposal + @$|\Pi|$@
    broadcast <Prepare | proposal>
    wait for a majority of <Prepared | ap, av>
    if any av returned, replace proposed_value with av with highest ap
    
accept():
    broadcast <Accept | proposal, proposed_value>
    wait for a majority of <Accepted | mp>
    if all mp <= proposal:
        decided = true
        trigger <Decide | proposed_value>

@\textbf{Acceptors execute:}
    min_proposal = 0
    accepted_proposal = 0
    accepted_value = @$\bot$@

upon <Prepare | proposal>:
    if proposal > min_proposal:
        min_proposal = n
    reply <Prepared | accepted_proposal, accepted_value>

upon <Accept | proposal, value>:
    if proposal >= min_proposal:
        accepted_proposal = min_proposal = n
        accepted_value = value
    reply <Accepted | min_proposal>
\end{lstlisting}
